Energy consumption of smartphones and IoT devices when using different versions of the HTTP protocol

HTTP is frequently used by smartphones and IoT devices to access information and Web services. Nowadays, HTTP is used in three major versions, each introducing significant changes with respect to the previous one. We evaluated the energy consumption of the major versions of the HTTP protocol when used in the communication between energy-constrained devices and cloud-based or edge-based services. Experimental results show that in a machine-to-machine communication scenario, for the considered client devices - a smartphone and a Single Board Computer - and for a number of cloud/edge services and facilities, HTTP/3 frequently requires more energy than the previous versions of the protocol. The focus of our analysis is on machine-to-machine communication, but to obtain a broader view we also considered a client-server interaction pattern that is more browsing-like. In this case, HTTP/3 can be more energy efficient than the other versions.

==> old/100K.tex <==
\section{100K}

\begin{figure}[!h]
    \centering
        \subfloat[Finestra crescente di dimentsion]{
            \includegraphics[width=0.9\textwidth]{Figures/100K/Perfasce_incrWindows_100K.pdf}
            %\label{}
        }
        \\
        \subfloat[anova1]{
            \includegraphics[width=0.3\textwidth]{Figures/100K/anova1_100000.pdf}
            %\label{}
        }
        \hspace{0.3cm}
        \subfloat[anova1 tabellato]{
            \includegraphics[width=0.4\textwidth]{Figures/100K/anova1_table.PNG}
            %\label{}
        }
        \\
        \subfloat[anova2 comparazione protocolli]{
            \includegraphics[width=0.49\textwidth]{Figures/100K/anova2_compareproto_100000.PNG}
            %\label{}
        }
        \subfloat[anova2 comparazione fasce]{
            \includegraphics[width=0.49\textwidth]{Figures/100K/anova2_comparefascia_100000.PNG}
            %\label{}
        }\\
        \subfloat[anova2 tabellato]{
            \includegraphics[width=0.4\textwidth]{Figures/100K/anova2_100000.png}
            %\label{}
        }
        \subfloat[media delle fasce]{
            \includegraphics[width=0.6\textwidth]{Figures/100K/MediadelleFasce_100000fig.png}
            %\label{}
        }
       
        \caption{Payload = 100000 carateri}
        \label{fig:XX}
\end{figure}
\begin{figure}[!h]
    \centering
        \subfloat[Response code]{
            \includegraphics[width=0.99\textwidth]{Figures/100K/colo_100000chars.png}
            %\label{}
        }
                \caption{Payload = 100000 carateri}
        \label{fig:XX}
\end{figure}



\begin{figure}[!h]
    \centering
        \subfloat[http11]{
            \includegraphics[width=0.45\textwidth]{Figures/100K/regressioneHTTP11_100000.png}
            %\label{}
        }
        \subfloat[http11 - tabella]{
            \includegraphics[width=0.45\textwidth]{Figures/100K/regressioneHTTP11_100000_tabella.png}
            %\label{}
        }\\
        \subfloat[http2]{
            \includegraphics[width=0.45\textwidth]{Figures/100K/regressioneHTTP2_100000.png}
            %\label{}
        }
        \subfloat[http2 - tabella]{
            \includegraphics[width=0.45\textwidth]{Figures/100K/regressioneHTTP2_100000_tabella.png}
            %\label{}
        }\\
        \subfloat[http3]{
            \includegraphics[width=0.45\textwidth]{Figures/100K/regressioneHTTP3_100000.png}
            %\label{}
        }
        \subfloat[http3 - tabella]{
            \includegraphics[width=0.45\textwidth]{Figures/100K/regressioneHTTP3_100000_tabella.png}
            %\label{}
        }\\
       
        \caption{Regressione Payload = 100000 carateri}
        \label{fig:XX}
\end{figure}


==> old/1024K.tex <==
\section{1024K}

\begin{figure}[!h]
    \centering
        \subfloat[Finestra crescente di dimentsion]{
            \includegraphics[width=0.9\textwidth]{Figures/1024K/Perfasce_incrWindows_1024K.png}
            %\label{}
        }
        \\
        \subfloat[anova1]{
            \includegraphics[width=0.3\textwidth]{Figures/1024K/anova1_1024.png}
            %\label{}
        }
        \hspace{0.3cm}
        \subfloat[anova1 tabellato]{
            \includegraphics[width=0.4\textwidth]{Figures/1024K/anova1_table_1024.PNG}
            %\label{}
        }
        \\
        \subfloat[anova2 comparazione protocolli]{
            \includegraphics[width=0.49\textwidth]{Figures/1024K/anova2_compareproto_1024000.PNG}
            %\label{}
        }
        \subfloat[anova2 comparazione fasce]{
            \includegraphics[width=0.49\textwidth]{Figures/1024K/anova2_comparefascia_1024000.PNG}
            %\label{}
        }\\
        \subfloat[anova2 tabellato]{
            \includegraphics[width=0.4\textwidth]{Figures/1024K/anova2_1024000.png}
            %\label{}
        }
        \subfloat[media delle fasce]{
            \includegraphics[width=0.6\textwidth]{Figures/1024K/MediadelleFasce_1024000fig.png}
            %\label{}
        }
       
        \caption{Payload = 1024000 carateri}
        \label{fig:XX}
\end{figure}


\begin{figure}[!h]
    \centering
        \subfloat[Response code]{
            \includegraphics[width=0.99\textwidth]{Figures/1024K/colo_1024000chars.png}
            %\label{}
        }
                \caption{Payload = 1024000 carateri}
        \label{fig:XX}
\end{figure}

==> old/1024K_2.tex <==
\section{1024K}

\begin{figure}[!h]
    \centering
        \subfloat[scatter]{
            \includegraphics[width=0.4\textwidth]{Figures/1024K_2/scatter.png}
        }
        \\
        \subfloat[anovan tutti]{
            \includegraphics[width=0.5\textwidth]{Figures/1024K_2/anovan_0_1.PNG}
        }
        \\
        \subfloat[anovan tutti]{
            \includegraphics[width=0.3\textwidth]{Figures/1024K_2/anovan_0_1_comparepf.png}
        }
        \subfloat[anovan tutti]{
            \includegraphics[width=0.3\textwidth]{Figures/1024K_2/anovan_0_1_compareps.png}
        }
        \subfloat[anovan tutti]{
            \includegraphics[width=0.3\textwidth]{Figures/1024K_2/anovan_0_1_comparesf.png}
        }
       \\
       \subfloat[anova1 e-p - MRS]{
            \includegraphics[width=0.48\textwidth]{Figures/1024K_2/anova1_0_ep.PNG}
        }
        \subfloat[anova1 - es - MRS]{
            \includegraphics[width=0.48\textwidth]{Figures/1024K_2/anova1_0_es.PNG}
        }
        \\
       \subfloat[anova1 e-p - MXP]{
            \includegraphics[width=0.48\textwidth]{Figures/1024K_2/anova1_1_ep.PNG}
        }
        \subfloat[anova1 - es - MXP]{
            \includegraphics[width=0.48\textwidth]{Figures/1024K_2/anova1_1_es.PNG}
        }
        \caption{Payload = 1024000 carateri}
        \label{fig:XX}
\end{figure}




==> old/1024K_3.tex <==
\section{1024K - 3}

\begin{figure}[!h]
    \centering
        \subfloat[Response code]{
            \includegraphics[width=0.99\textwidth]{Figures/1024K_3/colo_1024000chars.png}
            %\label{}
        }
                \caption{Payload = 1024000 carateri}
        \label{fig:XX}
\end{figure}

\begin{figure}[!h]
    \centering
        \subfloat[Incr. window]{
            \includegraphics[width=0.99\textwidth]{Figures/1024K_3/Energy_incrWindow.png}
            %\label{}
        }
                \caption{Payload = 1024000 carateri}
        \label{fig:XX}
\end{figure}



\begin{figure}[!h]
    \centering
    \subfloat[anova 1 (proto) - facility 0 (MRS)]{
        \includegraphics[width=0.4\textwidth]{Figures/1024K_3/anova1_0_ep_tabella.PNG}
    }
    \subfloat[anova 1 (proto) - facility 0 (MRS)]{
        \includegraphics[width=0.35\textwidth]{Figures/1024K_3/anova1_0_ep_boxplot.PNG}
    }
    \\
    
    \subfloat[anova 1 (slot) - facility 0 (MRS)]{
        \includegraphics[width=0.4\textwidth]{Figures/1024K_3/anova1_0_es_tabella.PNG}
    }
    \subfloat[anova 1 (slot) - facility 0 (MRS)]{
        \includegraphics[width=0.35\textwidth]{Figures/1024K_3/anova1_0_es_boxplot.PNG}
    }
    \\
    
    \subfloat[anova 1 (proto) - facility 1(MXP)]{
        \includegraphics[width=0.4\textwidth]{Figures/1024K_3/anova1_1_ep_tabella.PNG}
    }
    \subfloat[anova 1 (proto) - facility 1 (MXP)]{
        \includegraphics[width=0.4\textwidth]{Figures/1024K_3/anova1_1_ep_boxplot.PNG}
    }
    \\
    
    \subfloat[anova 1 (slot) - facility 1 (MXP)]{
        \includegraphics[width=0.4\textwidth]{Figures/1024K_3/anova1_1_es_tabella.PNG}
    }
    \subfloat[anova 1 (slot) - facility 1 (MXP)]{
       \includegraphics[width=0.4\textwidth]{Figures/1024K_3/anova1_1_es_boxplot.PNG}
    }
    
    \caption{Anova 1- Payload = 1024000 carateri}
    \label{fig:XX}
\end{figure}




\begin{figure}[!h]
    \centering
        \subfloat[anova 1 (proto)]{
            \includegraphics[width=0.4\textwidth]{Figures/1024K_3/anova1_ep_tabella.PNG}
        }
        \subfloat[anova 1 (proto)]{
            \includegraphics[width=0.35\textwidth]{Figures/1024K_3/anova1_ep_boxplot.PNG}
        }
        \\
        
        \subfloat[anova 1 (slot)]{
            \includegraphics[width=0.4\textwidth]{Figures/1024K_3/anova1_es_tabella.PNG}
        }
        \subfloat[anova 1 (slot)]{
            \includegraphics[width=0.35\textwidth]{Figures/1024K_3/anova1_es_boxplot.PNG}
        }
        
        \caption{Anova 1- Payload = 1024000 carateri}
        \label{fig:XX}
\end{figure}



\begin{figure}[!h]
    \centering
    \subfloat[anova n (proto - slot) - facility 0 (MRS)]{
        \includegraphics[width=0.4\textwidth]{Figures/1024K_3/anovan_0_ps_tabella.PNG}
    }
    \subfloat[anova n (proto - slot) - facility 0 (MRS)]{
        \includegraphics[width=0.35\textwidth]{Figures/1024K_3/anovan_0_ps_multcompare.PNG}
    }
    \\
 
    
    \subfloat[anova n (proto - slot) -facility 1(MXP)]{
        \includegraphics[width=0.4\textwidth]{Figures/1024K_3/anovan_1_ps_tabella.PNG}
    }
    \subfloat[anova n (proto - slot) -facility 1 (MXP)]{
        \includegraphics[width=0.4\textwidth]{Figures/1024K_3/anovan_1_ps_multcompare.PNG}
    }
    \\
    
    \subfloat[anova n (proto - slot)]{
        \includegraphics[width=0.4\textwidth]{Figures/1024K_3/anovan_ps_tabella.PNG}
    }
    \subfloat[anova n (proto - slot)]{
        \includegraphics[width=0.4\textwidth]{Figures/1024K_3/anovan_ps_multcompare.PNG}
    }
    \caption{Anovan - Payload = 1024000 carateri}
    \label{fig:XX}
\end{figure}



\begin{figure}[!h]
    \centering
    \subfloat[MRS]{
        \includegraphics[width=0.55\textwidth]{Figures/1024K_3/meanFasce_MRS.png}
    }
    \\
 
    
     \subfloat[MXP]{
        \includegraphics[width=0.55\textwidth]{Figures/1024K_3/meanFasce_MXP.png}
    }
    \\
    
    
     \subfloat[MRS + MXP]{
        \includegraphics[width=0.55\textwidth]{Figures/1024K_3/meanFasce.png}
    }
    \\
    \caption{Media delle energie}
    \label{fig:XX}
\end{figure}

==> old/2048K.tex <==
\section{2048K}

\begin{figure}[!h]
    \centering
        \subfloat[Response code]{
            \includegraphics[width=0.99\textwidth]{Figures/2048K/colo_2048000chars.png}
            %\label{}
        }
                \caption{Payload = 2048K carateri}
        \label{fig:XX}
\end{figure}

\begin{figure}[!h]
    \centering
        \subfloat[Incr. window]{
            \includegraphics[width=0.99\textwidth]{Figures/2048K/Energy_incrWindow.png}
            %\label{}
        }
                \caption{Payload = 2048K carateri}
        \label{fig:XX}
\end{figure}



\begin{figure}[!h]
    \centering
   % \subfloat[anova 1 (proto) - facility 0 (MRS)]{
    %    \includegraphics[width=0.25\textwidth]{Figures/2048K/anova1_0_ep_tabella.PNG}
    %}
    %\subfloat[anova 1 (proto) - facility 0 (MRS)]{
    %    \includegraphics[width=0.25\textwidth]{Figures/2048K/anova1_0_ep_boxplot.PNG}
    %}
    %\\
    
    %\subfloat[anova 1 (slot) - facility 0 (MRS)]{
    %    \includegraphics[width=0.25\textwidth]{Figures/2048K/anova1_0_es_tabella.PNG}
    %}
    %\subfloat[anova 1 (slot) - facility 0 (MRS)]{
    %    \includegraphics[width=0.25\textwidth]{Figures/2048K/anova1_0_es_boxplot.PNG}
    %}
    %\\
    
    \subfloat[anova 1 (proto) - facility 1(MXP)]{
        \includegraphics[width=0.4\textwidth]{Figures/2048K/anova1_1_ep_tabella.png}
    }
    \subfloat[anova 1 (proto) - facility 1 (MXP)]{
        \includegraphics[width=0.4\textwidth]{Figures/2048K/anova1_1_ep_boxplot.png}
    }
    \\
    
    \subfloat[anova 1 (slot) - facility 1 (MXP)]{
        \includegraphics[width=0.4\textwidth]{Figures/2048K/anova1_1_es_tabella.png}
    }
    \subfloat[anova 1 (slot) - facility 1 (MXP)]{
       \includegraphics[width=0.4\textwidth]{Figures/2048K/anova1_1_es_boxplot.png}
    }
    
    \caption{Anova 1- Payload = 2048K carateri}
    \label{fig:XX}
\end{figure}




\begin{figure}[!h]
    \centering
        \subfloat[anova 1 (proto)]{
            \includegraphics[width=0.4\textwidth]{Figures/2048K/anova1_ep_tabella.png}
        }
        \subfloat[anova 1 (proto)]{
            \includegraphics[width=0.35\textwidth]{Figures/2048K/anova1_ep_boxplot.png}
        }
        \\
        
        \subfloat[anova 1 (slot)]{
            \includegraphics[width=0.4\textwidth]{Figures/2048K/anova1_es_tabella.png}
        }
        \subfloat[anova 1 (slot)]{
            \includegraphics[width=0.35\textwidth]{Figures/2048K/anova1_es_boxplot.png}
        }
        
        \caption{Anova 1- Payload = 2048K carateri}
        \label{fig:XX}
\end{figure}



\begin{figure}[!h]
    \centering
    %\subfloat[anova n (proto - slot) - facility 0 (MRS)]{
        %\includegraphics[width=0.4\textwidth]{Figures/2048K/anovan_0_ps_tabella.PNG}
   % }
    %\subfloat[anova n (proto - slot) - facility 0 (MRS)]{
        %\includegraphics[width=0.35\textwidth]{Figures/2048K/anovan_0_ps_multcompare.PNG}
    %}
    %\\
 
    
    \subfloat[anova n (proto - slot) -facility 1(MXP)]{
        \includegraphics[width=0.4\textwidth]{Figures/2048K/anovan_1_ps_tabella.png}
    }
    \subfloat[anova n (proto - slot) -facility 1 (MXP)]{
        \includegraphics[width=0.4\textwidth]{Figures/2048K/anovan_1_ps_multcompare.png}
    }
    \\
    
    \subfloat[anova n (proto - slot)]{
        \includegraphics[width=0.4\textwidth]{Figures/2048K/anovan_ps_tabella.png}
    }
    \subfloat[anova n (proto - slot)]{
        \includegraphics[width=0.4\textwidth]{Figures/2048K/anovan_ps_multcompare.png}
    }
    \caption{Anovan - Payload = 2048K carateri}
    \label{fig:XX}
\end{figure}



\begin{figure}[!h]
    \centering
    %\subfloat[MRS]{
        %\includegraphics[width=0.3
        %\textwidth]{Figures/2048K/meanFasce_MRS.png}
    %}
    %\\
 
    
     \subfloat[MXP]{
        \includegraphics[width=0.3\textwidth]{Figures/2048K/meanFasce_MXP.png}
    }
    \\
    
    
     \subfloat[MRS + MXP]{
        \includegraphics[width=0.55\textwidth]{Figures/2048K/meanFasce.png}
    }
    \\
    \caption{Media delle energie}
    \label{fig:XX}
\end{figure}

==> old/experimentalSetup.tex <==

\section{Experimental Setup - Chiara}
\label{sec:setup}

\begin{figure}[!tb]
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/clientserver_interaction.pdf}
    \caption{The communication schema between a client application running on an Android smartphne and an edge server.}
    \label{fig:client-serverInteraction}
\end{figure}

In this study, we evaluate the energy consumed by a device to interact with a edge server using multiple versions of the HTTP protocol, in particular HTTP 1.1, 2, and 3.


The device operates according to a client-server paradigm, issuing periodic requests to an edge server, as illustrated in Figure~\ref{fig:client-serverInteraction}. At the beginning of each period, the client sends a HTTP request. The server then sends a HTTP reply as soon as possible. When the HTTP reply is entirely received, the client waits until the start of the next period. In our experiments we used two types of devices, an Android Nexus 5 smartphone with Android 6 OS, and a Raspberry Pi XXX device with XXX OS. To measure the power consumption on the devices, we used a Qoitech Otii external power analyzer~\cite{otii}, capable of collecting current, voltage, and power consumption metrics. The power analyzer also acts as a power supply for the connected device. This can be particularly challenging in the smartphone case. To connect the power analyzer to the smartphone we had to make some modifications to the smartphone. We removed the battery from the smartphone, and we separated the cells from the battery control circuit. Then, we soldered two connectors directly on the circuitry. These connectors are used for connecting the smartphone and the power monitor. To compensate for any voltage drop at the input of the smartphone, we soldered 7 ceramic capacitors of 100 $\mu$F each in parallel as close as possible to the circuit. Finally, we reconnected the modified circuit to the smartphone motherboard.


We measured the energy consumption of a client application interacting with an edge server using the HTTP protocol. The client application was executed on an Android smartphone on a periodical basis. 
The client-server communication schema is illustrated in Figure \ref{fig:client-serverInteraction}. 
At the beginning of each period, the client sends to the server an HTTP POST request using $s$ bytes of payload. The payload of the first request is generated completely randomly, while only the first 40 bytes of the following request are rewritten. This allows limiting the use of computational resources in the presence of large payloads as only a few bytes are generated at each period. At the same time, it guarantees a different payload to each request, inhibiting any caching mechanisms that can be present along the path.
The server starts processing incoming requests as soon as possible. To limit the server-side processing time, the request payload is used also for the response without any modification.



\begin{figure}[!tb]
    \centering
    \includegraphics[width=0.48\textwidth]{Figures/setup.pdf}
    \caption{The setup used during the experimental phase.}
    \label{fig:experimetalSetup}
\end{figure}
We performed a set of experiments considering different versions of HTTP and different payload sizes ($s$). 
The client application was executed on a Nexus 5 with Android 6 OS. The smartphone was connected to the LTE network of a well-known Italian operator. 
To measure the consumption of the client we used an external power analyzer capable of collecting current, voltage, and power consumption metrics. Additionally, the selected appliance works also as a power supply for the smartphone. 
To connect the power monitor and the smartphone we have made some modifications to the smartphone. Precisely, we removed the battery from the smartphone, and we separated the cells from the battery control circuit. Then, we soldered directly on the circuitry two connectors. Basically, the connectors are used for connecting the smartphone and the power monitor. 
To compensate for any voltage drop at the input of the smartphone, we soldered in parallel as close as possible to the circuit 7 ceramic capacitors of 100 $\mu$F each. 
Finally, the modified circuit was reconnected to the smartphone motherboard.  
Instead, the server was executed using the Cloudflare worker service, which allows serverless functions to be run in one of the 270 Cloudflare data centers~\cite{cloudflare-worker}. Cloudflare does not allow selecting the facility. The latter is automatically chosen on the basis of a proximity criterion, thus it should be the closest one~\cite{clouflare-facility}.

In order to assess the energy consumption of our application, it is necessary to consider the impact that third-party applications might have on the consumption of the entire device. For this purpose, before the beginning of the experimental phase, we performed a factory reset of the device. After that, we removed all the pre-installed apps. Unfortunately, there are a small number of apps that could not be removed. For them, we disabled the possibility of using the network when in the background. 
\\**************\\
Instead, during the second round of experiments, we studied the smartphone when communicating with an object storage service.
This service, named Google Cloud Storage (GCS), allows users to retrieve files from buckets hosted on Google servers via the HTTP protocol.
Basically, the client application periodically sends an HTTP GET request on a regular basis, downloading a given resource from the target bucket. To prevent any potential caching mechanism, at each step, the client asks for a different resource. To assess the impact of the latency, we set up three distinct buckets located in Milan (edge), South Carolina (cloud), and Melbourne (far cloud).
\\**************\\



==> old/non-serve-piu.tex <==

\section{Results}

We first present the results obtained with the smartphone and then the results obtained with the SBC. 

\subsection{Smartphone-Cloudflare}

We considered the following values for the size $s$ of the payload in requests and replies: 400, 1024, and 2048 kB. The period between consecutive requests was set to 20 s. 



%The first one is hosted in Milan, while the second is located in Marseille. Both are reasonably close to the location where the client was placed (Pisa, Italy). Cloudflare specifies that any request exceeding the first one is handled by the nearest facility. The two facilities are subjected to different network conditions since they are located in different countries and are placed at different distances from the client. Hence, we decided to divide the results into two different sets, one per facility. Finally, we discarded the results of the experiments during which the facility was subject to changes. It is important to notice that the facility handling a request cannot be selected by the experimenters, and it is instead automatically chosen by Cloudflare. We preferred to remove the results of these experiments to have reasonably stable network conditions during the whole 1-hour experiments. 

For each 1-hour experiment, we processed the metrics collected by the power analyzer as follows. First, we divided the results of the experiments into 10 slots of equal size. Thus, each slot contains 6 minutes of measurements. Next, for each of these slots, we calculated the average consumption. Figure \ref{fig:Energy_1024} shows a 1-hour experiment, where each curve corresponds to the energy needed by a different version of the HTTP protocol. Points represent the average energy consumption during the considered 6-minute slot. Even though the behavior of the client application does not change during the experiment, some fluctuations can be observed in the amount of needed energy. Such fluctuations are due to changing network conditions and the possibly different load on the edge infrastructure. 


\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\textwidth]{Figures/ultimi/1024K/Power.pdf}
    
    \caption{The energy consumption of the smartphone when interacting with the serverless edge infrastructure; payload size ($s$) is equal to 1024 kB.}
    \label{fig:Energy_1024}
\end{figure}   

\begin{comment} 
 \begin{figure*}[!h]
    \centering
    
    \subfloat[Cloudflare facility code MXP (Milan)]{
        \includegraphics[width=0.4\textwidth]{Figures/Results/Anova1/MXP_e-p.png}
        \label{fig:anova1_1024_proto_milan}
    }
    \hspace{1cm}
    \subfloat[Cloudflare facility code MRS (Marseille)]{
        \includegraphics[width=0.4\textwidth]{Figures/Results/Anova1/MRS_e-p_merged.png}
        \label{fig:anova1_1024_proto_marseille}
    }
    \caption{The impact of the HTTP version on the energy consumption of the smartphones. The results refers to the set of experiments using a payload of 1024000 characters. For each boxplot, the red mark indicates the median value, the upper and the lower borders show the 25th and 75th percentiles, and finally the whiskers confine all the values in the [$q_3 + 1.5 \cdot IQR$, $q_1 - 1.5 \cdot IQR$] interval.}
    \label{fig:anova1_1024_proto}
\end{figure*}
\end{comment}

\begin{table}[]
    \centering
                \begin{tabular}{rrr}
                    \toprule
                     s  & p-value (Version) & p-value (ToD)\\
                     \hline
                     400K  & 0.0025    & 0.0202    \\
                     1024K & 0         & 0.6517    \\
                     2048K & 0.0027    & 0.0072    \\
                     \bottomrule
                \end{tabular}
    \caption{p values for the different experiments}
    \label{tab:pvalues}
\end{table}

\begin{figure*}[!h]
    \centering
        \subfloat[400K, MXP]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/400K/MXP_anovan_e-ps.pdf}
        }
        \subfloat[1024K, MRS]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/1024K/MRS_anovan_e-ps.pdf}
        }
        \\
        \subfloat[1024K, MXP]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/1024K/MXP_anovan_e-ps.pdf}
            \label{subfig:1024}
        }
        \subfloat[2048K, MXP]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/2048K/MXP_anovan_e-ps.pdf}
        }
        
        \caption{ANOVAN, protocol Version and ToD are the explanatory variables, power consumption is the dependent variable.}
        \label{fig:nexus-cloudflare-anovan}
\end{figure*}

Then we performed an  analysis of variance (ANOVAN) where we considered the Time of the Day (ToD) and the version of the protocol as explanatory variables and the power consumption as the dependent variable.  
%Figure \ref{fig:nexus-cloudflare-anovan} shows the comparison for different values of $s$. Results are grouped by the protocol version (1, 2, and 3 to respectively indicate HTTP 1.1, HTTP 2, and HTTP 3) and ToD. Results with the same ToD value have been obtained at the same time of the day. The ToD values are different for the considered payload $s$ values because, as mentioned, the facility cannot be selected by us and it can be changed during an experiment, forcing us to discard many runs. In summary, the analysis has been restricted to the ToD values for which we were able to collect an entire hour of data for all the three versions of HTTP.  

Table \ref{tab:pvalues} shows the p-value resulting from the ANOVAN analysis. The version of the protocol is always significant in explaining the different average values of the energy consumption. This is also visible, for instance, in Figure~\ref{subfig:1024}, where for the three ToD values (1, 2, 6), the average power consumption of HTTP 3 is higher than the other two versions. Overall, the HTTP 3 needs XXX-YYY\% more energy than the previous versions of the protocol, with the largest additional energy needed when the payload is larger. 

%As can be seen, the energy consumption metrics are less variable when the requests are processed in Milan. In fact, the boxplots in Figure \ref{fig:anova1_1024_proto_milan} are shorter than those in Figure \ref{fig:anova1_1024_proto_marseille}.  
%Additionally, when HTTP 1.1 and HTTP2 protocols are involved the median value is smaller when the 


\begin{figure*}[!h]
    \centering
        \subfloat[raspberry, 1024K, MXP]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/raspberry_1024K/MXP_anovan_e-ps.pdf}
        }
        \\
    
        \subfloat[raspberry, 2048K, MXP]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/raspberry_2048K/MXP_anovan_e-ps.pdf}
        }
        \subfloat[raspberry, 4096K, MXP]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/raspberry_4096K/MXP_anovan_e-ps.pdf}
        }
        
        \caption{ANOVAN, protocol Version and ToD are the explanatory variables, power consumption is the dependent variable.}
        \label{fig:raspberry-cloudflare-anovan}
\end{figure*}


\begin{figure*}[!h]
    \centering
        \subfloat[XXXDACONTROLLAREXXXsmartphone]{
            \includegraphics[width=0.49\textwidth]{Figures/ultimi/anocova/smartphone/no_outlier.pdf}
        }
        \subfloat[XXXDARIMUOVEREXXXraspberry zero]{
            \includegraphics[width=0.49\textwidth]{Figures/ultimi/anocova/pi0Manual/no_outlier.pdf}
        }
        \\
        \subfloat[XXXDARIMUOVEREXXXraspberry Pi3 with automaticToolbox and outlier]{
            \includegraphics[width=0.49\textwidth]{Figures/ultimi/anocova/Pi3Automated/no_filtering.pdf}
        }\subfloat[XXXDARIMUOVEREXXXraspberry Pi3 with automaticToolbox and without outlier]{
            \includegraphics[width=0.49\textwidth]{Figures/ultimi/anocova/Pi3Automated/no_outlier.pdf}
        }
        \label{fig:raspberry_smartphone-cloudflare-anocova}
\end{figure*}

\begin{figure*}[!h]
    \centering
        \subfloat[raspberry- milano]{
            \includegraphics[width=0.48\textwidth]{results/GCS/Anocova-raspberryPi3/milano.png}
        }
        \subfloat[raspberry- londra]{
            \includegraphics[width=0.48\textwidth]{results/GCS/Anocova-raspberryPi3/londra.png}
        }
        \\
        \subfloat[raspberry- carolina]{
            \includegraphics[width=0.48\textwidth]{results/GCS/Anocova-raspberryPi3/carolina.png}
        }
        \subfloat[raspberry- melbourne]{
            \includegraphics[width=0.48\textwidth]{results/GCS/Anocova-raspberryPi3/melbourne}
        }
        \caption{Esperimenti raspberryPi3, automation toolbox, ultima versioni, giorni 03/01 + 09/01}
        \label{fig:anocova-GCS}
\end{figure*}
\begin{figure*}[!h]
    \centering
        \subfloat[raspberriPI3 - MXP]{
            \includegraphics[width=0.48\textwidth]{results/cloudflare/Anocova-RaspberryPi3/cloudflare_MXP.png}
        }
        
        \caption{Esperimenti raspberryPi3, automation toolbox, ultima versioni, giorni 10/01 - 11/01}
        \label{fig:anocova-GCS}
\end{figure*}
\begin{comment}
\begin{figure*}[!h]
    \centering
        \subfloat[smartphone]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/anocova/smartphone/no_outlier_multcompare.pdf}
        }
        \subfloat[raspberry]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/anocova/pi0Manual/no_outlier_multcompare.pdf}
        }
        \\
        \subfloat[raspberry Pi3 with automaticToolbox and outlier]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/anocova/Pi3Automated/no_filtering_multcompare.pdf}
        }
        \subfloat[raspberry Pi3 with automaticToolbox and without outlier]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/anocova/Pi3Automated/no_outlier_multcompare.pdf}
        }
        \caption{}
        \label{fig:raspberry_smartphone-cloudflare-anocova}
\end{figure*}
\end{comment}




\begin{figure}[!h]
    \centering
    \subfloat[Cloudflare facility code MRS (Marseille)]{
        \includegraphics[width=0.4\textwidth]{Figures/Results/Anova1/anova1_0_es.PNG}
    }
    \\
    
    

    \subfloat[Cloudflare facility code MXP (Milan)]{
       \includegraphics[width=0.4\textwidth]{Figures/Results/Anova1/anova1_1_es.PNG}
    }
    
    \caption{The impact of the slot on the energy consumption of the smartphones. The results refers to the set of experiments using a payload of 1024000 characters.}
    \label{fig:anova1_1024_slot}
\end{figure}






==> old/note.tex <==
\section{NOTE}
OUTPUT CURL  
\\\textbf{$->$ }certs Output the certificate chain with details. Supported only by the OpenSSL, GnuTLS, Schannel, NSS, GSKit and Secure Transport backends (Added in 7.88.0)
\\\textbf{$->$ }content\_type The Content-Type of the requested document, if there was any.
\\\textbf{$->$ }errormsg The error message. (Added in 7.75.0)
\\\textbf{$->$ }exitcode The numerical exitcode of the transfer. (Added in 7.75.0)
\\\textbf{$->$ }filename\_effective The ultimate filename that curl writes out to. This is only meaningful if curl is told to write to a file with the -O, --remote-name or -o, --output option. It's most useful in combination with the -J, --remote-header-name option.
\\\textbf{$->$ }ftp\_entry\_path The initial path curl ended up in when logging on to the remote FTP server.
\\\textbf{$->$ }header\_json A JSON object with all HTTP response headers from the recent transfer. Values are provided as arrays, since in the case of multiple headers there can be multiple values.
\\\textbf{$->$ }The header names provided in lowercase, listed in order of appearance over the wire. Except for duplicated headers. They are grouped on the first occurrence of that header, each value is presented in the JSON array.
\\\textbf{$->$ }http\_code The numerical response code that was found in the last retrieved HTTP(S) or FTP(s) transfer.
\\\textbf{$->$ }http\_connect The numerical code that was found in the last response (from a proxy) to a curl CONNECT request.
\\\textbf{$->$ }http\_version The http version that was effectively used. (Added in 7.50.0)
\\\textbf{$->$ }json A JSON object with all available keys.
\\\textbf{$->$ }local\_ip The IP address of the local end of the most recently done connection \\\textbf{$->$ }can be either IPv4 or IPv6.
\\\textbf{$->$ }local\_port The local port number of the most recently done connection.
\\\textbf{$->$ }method The http method used in the most recent HTTP request. (Added in 7.72.0)
\\\textbf{$->$ }num\_certs Number of server certificates received in the TLS handshake. Supported only by the OpenSSL, GnuTLS, Schannel, NSS, GSKit and Secure Transport backends (Added in 7.88.0)
\\\textbf{$->$ }num\_connects Number of new connects made in the recent transfer.
\\\textbf{$->$ }num\_headers The number of response headers in the most recent request (restarted at each redirect). Note that the status line IS NOT a header. (Added in 7.73.0)
\\\textbf{$->$ }num\_redirects Number of redirects that were followed in the request.
\\\textbf{$->$ }onerror The rest of the output is only shown if the transfer returned a non-zero error (Added in 7.75.0)
\\\textbf{$->$ }proxy\_ssl\_verify\_result The result of the HTTPS proxy's SSL peer certificate verification that was requested. 0 means the verification was successful. (Added in 7.52.0)
\\\textbf{$->$ }redirect\_url When an HTTP request was made without -L, --location to follow redirects (or when --max-redirs is met), this variable will show the actual URL a redirect would have gone to.
\\\textbf{$->$ }referer The Referer: header, if there was any. (Added in 7.76.0)
\\\textbf{$->$ }remote\_ip The remote IP address of the most recently done connection \\\textbf{$->$ }can be either IPv4 or IPv6.
\\\textbf{$->$ }remote\_port The remote port number of the most recently done connection.
\\\textbf{$->$ }response\_code The numerical response code that was found in the last transfer (formerly known as "http\_code").
\\\textbf{$->$ }scheme The URL scheme (sometimes called protocol) that was effectively used. (Added in 7.52.0)
\\\textbf{$->$ }size\_download The total amount of bytes that were downloaded. This is the size of the body/data that was transferred, excluding headers.
\\\textbf{$->$ }size\_header The total amount of bytes of the downloaded headers.
\\\textbf{$->$ }size\_request The total amount of bytes that were sent in the HTTP request.
\\\textbf{$->$ }size\_upload The total amount of bytes that were uploaded. This is the size of the body/data that was transferred, excluding headers.
\\\textbf{$->$ }speed\_download The average download speed that curl measured for the complete download. Bytes per second.
\\\textbf{$->$ }speed\_upload The average upload speed that curl measured for the complete upload. Bytes per second.
\\\textbf{$->$ }ssl\_verify\_result The result of the SSL peer certificate verification that was requested. 0 means the verification was successful.
\\\textbf{$->$ }stderr From this point on, the -w, --write-out output will be written to standard error. (Added in 7.63.0)
\\\textbf{$->$ }stdout From this point on, the -w, --write-out output will be written to standard output. This is the default, but can be used to switch back after switching to stderr. (Added in 7.63.0)
\\\textbf{$->$ }time\_appconnect The time, in seconds, it took from the start until the SSL/SSH/etc connect/handshake to the remote host was completed.
\\\textbf{$->$ }time\_connect The time, in seconds, it took from the start until the TCP connect to the remote host (or proxy) was completed.
\\\textbf{$->$ }time\_namelookup The time, in seconds, it took from the start until the name resolving was completed.
\\\textbf{$->$ }time\_pretransfer The time, in seconds, it took from the start until the file transfer was just about to begin. This includes all pre-transfer commands and negotiations that are specific to the particular protocol(s) involved.
\\\textbf{$->$ }time\_redirect The time, in seconds, it took for all redirection steps including name lookup, connect, pretransfer and transfer before the final transaction was started. time\_redirect shows the complete execution time for multiple redirections.
\\\textbf{$->$ }time\_starttransfer The time, in seconds, it took from the start until the first byte was just about to be transferred. This includes time\_pretransfer and also the time the server needed to calculate the result.
\\\textbf{$->$ }time\_total The total time, in seconds, that the full operation lasted.
\\\textbf{$->$ }url The URL that was fetched. (Added in 7.75.0)
\\\textbf{$->$ }urlnum The URL index number of this transfer, 0-indexed. De-globbed URLs share the same index number as the origin globbed URL. (Added in 7.75.0)
\\\textbf{$->$ }url\_effective The URL that was fetched last. This is most meaningful if you have told curl to follow location: headers.


==> old/old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FINE ARTICOLO %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage

\input{note}

\begin{figure*}[!t]
    \centering
    \subfloat[idle]{
    \includegraphics[width=0.48\textwidth]{results/cloudflare/cpuOut/Cloudflare_idleCPU.png}
    }
    \subfloat[idle nooutliers]{
    \includegraphics[width=0.48\textwidth]{results/cloudflare/cpuOut/Cloudflare_idleCPU_nooutliers.png}}
    \\
    \subfloat[user]{
    \includegraphics[width=0.48\textwidth]{results/cloudflare/cpuOut/Cloudflare_userCPU.png}
    }
    \subfloat[user nooutliers]{
    \includegraphics[width=0.48\textwidth]{results/cloudflare/cpuOut/Cloudflare_userCPU_nooutliers.png}}\\
    \subfloat[system]{
    \includegraphics[width=0.48\textwidth]{results/cloudflare/cpuOut/Cloudflare_systemCPU.png}
    }
    \subfloat[system nooutliers]{
    \includegraphics[width=0.48\textwidth]{results/cloudflare/cpuOut/Cloudflare_systemCPU_nooutliers.png}}
    \\
    \subfloat[system + user]{
    \includegraphics[width=0.48\textwidth]{results/cloudflare/cpuOut/Cloudflare_systemUserCPU.png}
    }
    \subfloat[system nooutliers]{
    \includegraphics[width=0.48\textwidth]{results/cloudflare/cpuOut/Cloudflare_systemUserCPU_nooutliers.png}}
    \caption{User time cloudflare}
    \label{fig:cloudflareusertime}
\end{figure*}



\begin{figure*}[t]
    \centering
    \subfloat[speed upload]{
            \includegraphics[width=0.45\textwidth]{results/cloudflare/Cloudflare_sppedupload.png}
    }
    \subfloat[speed upload nooutliers]{
            \includegraphics[width=0.45\textwidth]{results/cloudflare/Cloudflare_sppedupload_nooutliers.png}
    }
    \\
    \subfloat[speed download]{
            \includegraphics[width=0.45\textwidth]{results/cloudflare/Cloudflare_sppeddownload.png}

    }
    \subfloat[speed download nooutliers]{
            \includegraphics[width=0.45\textwidth]{results/cloudflare/Cloudflare_sppeddownload_nooutliers.png}

    }
    \\
    \subfloat[timeappconnect]{
            \includegraphics[width=0.45\textwidth]{results/cloudflare/Cloudflare_timeappconnect.png}

    }
    \subfloat[timeappconnect nooutliers]{
            \includegraphics[width=0.45\textwidth]{results/cloudflare/Cloudflare_timeappconnect_nooutliers.png}

    }
    \\
    \subfloat[timeconnect]{
            \includegraphics[width=0.45\textwidth]{results/cloudflare/Cloudflare_timeconnect.png}

    }
    \subfloat[timeconnect nooutliers]{
            \includegraphics[width=0.45\textwidth]{results/cloudflare/Cloudflare_timeconnect_nooutliers.png}

    }
 \caption{Cloudflare - curl output}
    \label{fig:Cloudflare-TimeTotal}

 \end{figure*}

\begin{figure*}[t]
    \centering
    \subfloat[time name lookup]{
            \includegraphics[width=0.45\textwidth]{results/cloudflare/Cloudflare_timenamelookup.png}

    }
    \subfloat[time name lookup nooutliers]{
            \includegraphics[width=0.45\textwidth]{results/cloudflare/Cloudflare_timenamelookup_nooutliers.png}

    }
    \\
    \subfloat[time pretransfer]{
        \includegraphics[width=0.45\textwidth]{results/cloudflare/Cloudflare_timepretransfer.png}

    }
    \subfloat[time pretransfer nooutliers]{
        \includegraphics[width=0.45\textwidth]{results/cloudflare/Cloudflare_timepretransfer_nooutliers.png}

    }
    \\
    \subfloat[time starttransfer]{
            \includegraphics[width=0.45\textwidth]{results/cloudflare/Cloudflare_timestarttransfer.png}

    }
    \subfloat[time starttransfer nooutliers]{
            \includegraphics[width=0.45\textwidth]{results/cloudflare/Cloudflare_timestarttransfer_nooutliers.png}

    }
    \\
    \subfloat[time  total Cloudflare]{
            \includegraphics[width=0.45\textwidth]{results/cloudflare/Cloudflare_timetotal.png}

    }
    \subfloat[time  total Cloudflare nooutliers]{
            \includegraphics[width=0.45\textwidth]{results/cloudflare/Cloudflare_timetotal_nooutliers.png}

    }
    \caption{Cloudflare - curl output, parte 2}
    \label{fig:Cloudflare-TimeTotal2}
 \end{figure*}
 
 \begin{figure*}[!t]
    \centering
    \subfloat[ idle]{
            \includegraphics[width=0.45\textwidth]{results/GCS/cpuOut/GCS_idleCPU.png}
    }
    \subfloat[idle no outliers]{
            \includegraphics[width=0.45\textwidth]{results/GCS/cpuOut/GCS_idleCPU_nooutliers.png}
    }
    \\
    \subfloat[ User]{
            \includegraphics[width=0.45\textwidth]{results/GCS/cpuOut/GCS_userCPU.png}
    }
    \subfloat[ user no outliers]{
            \includegraphics[width=0.45\textwidth]{results/GCS/cpuOut/GCS_userCPU_nooutliers.png}
    }
    \\
    \subfloat[ system]{
            \includegraphics[width=0.45\textwidth]{results/GCS/cpuOut/GCS_systemCPU.png}
    }
    \subfloat[ system no outliers]{
            \includegraphics[width=0.45\textwidth]{results/GCS/cpuOut/GCS_systemCPU_nooutliers.png}
    }
    \\
    \subfloat[user + system]{
            \includegraphics[width=0.45\textwidth]{results/GCS/cpuOut/GCS_systemUserCPU.png}
    }
    \subfloat[user + system no outliers]{
            \includegraphics[width=0.45\textwidth]{results/GCS/cpuOut/GCS_systemUserCPU_nooutliers.png}
    }
    \caption{CPU time Google}
    \label{fig:GCSusertime}
\end{figure*}


\begin{figure*}[t]
    \centering
    \subfloat[speed upload]{
            \includegraphics[width=0.49\textwidth]{results/GCS/curlOut/GCS_sppedupload.png}
    }
    \subfloat[speed upload nooutliers]{
            \includegraphics[width=0.49\textwidth]{results/GCS/curlOut/GCS_sppedupload_nooutliers.png}
    }
    \\
    \subfloat[speed download]{
            \includegraphics[width=0.49\textwidth]{results/GCS/curlOut/GCS_sppeddownload.png}

    }
    \subfloat[speed download nooutliers]{
            \includegraphics[width=0.49\textwidth]{results/GCS/curlOut/GCS_sppeddownload_nooutliers.png}

    }
    \\
    \subfloat[timeappconnect]{
            \includegraphics[width=0.49\textwidth]{results/GCS/curlOut/GCS_timeappconnect.png}

    }
    \subfloat[timeappconnect nooutliers]{
            \includegraphics[width=0.49\textwidth]{results/GCS/curlOut/GCS_timeappconnect_nooutliers.png}

    }
 \caption{GCS - curl output}
    \label{fig:GCS-TimeTotal}

 \end{figure*}



\begin{figure*}[t]
    \centering
    
    \subfloat[timeconnect]{
            \includegraphics[width=0.49\textwidth]{results/GCS/curlOut/GCS_timeconnect.png}
    }
    \subfloat[timeconnect nooutliers]{
            \includegraphics[width=0.49\textwidth]{results/GCS/curlOut/GCS_timeconnect_nooutliers.png}
    }
    \\
    \subfloat[time name lookup]{
            \includegraphics[width=0.49\textwidth]{results/GCS/curlOut/GCS_timenamelookup.png}

    }
    \subfloat[time name lookup nooutliers]{
            \includegraphics[width=0.49\textwidth]{results/GCS/curlOut/GCS_timenamelookup_nooutliers.png}

    }
    \\
    \subfloat[time pretransfer]{
        \includegraphics[width=0.49\textwidth]{results/GCS/curlOut/GCS_timepretransfer.png}

    }
    \subfloat[time pretransfer nooutliers]{
        \includegraphics[width=0.49\textwidth]{results/GCS/curlOut/GCS_timepretransfer_nooutliers.png}

    }
 \caption{GCS - curl output, part 2}
    \label{fig:GCS-TimeTotal}

 \end{figure*}

\begin{figure*}[t]
    \centering
    \subfloat[time starttransfer]{
            \includegraphics[width=0.49\textwidth]{results/GCS/curlOut/GCS_timestarttransfer.png}

    }
    \subfloat[time starttransfer nooutliers]{
            \includegraphics[width=0.49\textwidth]{results/GCS/curlOut/GCS_timestarttransfer_nooutliers.png}

    }
    \\
    \subfloat[time  total Cloudflare]{
            \includegraphics[width=0.49\textwidth]{results/GCS/curlOut/GCS_timetotal.png}

    }
    \subfloat[time  total Cloudflare nooutliers]{
            \includegraphics[width=0.49\textwidth]{results/GCS/curlOut/GCS_timetotal_nooutliers.png}

    }
    \caption{GCS - curl output, parte 3}
    \label{fig:GCS-TimeTotal2}
 \end{figure*}


\newgeometry{left=0.2in,
            right=0.2in,
            top=0.2in,
            bottom=0.2in}
\onecolumn
\newpage


\begin{figure*}[!h]
    \centering
        \subfloat[]{
            \includegraphics[width=0.5\textwidth]{Figures/ultimi/100K/MXP_anovan_e-ps_tabella.png}
        }
        \subfloat[100K]{
            \includegraphics[width=0.2\textwidth]{Figures/ultimi/100K/anovan_e-ps.png}
        }
        \\\subfloat[]{
            \includegraphics[width=0.45\textwidth]{Figures/ultimi/400K/MXP_anovan_e-ps_tabella.pdf}
        }
        \subfloat[400K]{
            \includegraphics[width=0.55\textwidth]{Figures/ultimi/400K/MXP_anovan_e-ps.pdf}
        }
        \\
         \subfloat[]{
            \includegraphics[width=0.45\textwidth]{Figures/ultimi/1024K/MXP_anovan_e-ps_tabella.pdf}
        }
        \subfloat[1024K]{
            \includegraphics[width=0.55\textwidth]{Figures/ultimi/1024K/MXP_anovan_e-ps.pdf}
        }
        \\
        
        
        \subfloat[]{
            \includegraphics[width=0.45\textwidth]{Figures/ultimi/2048K/MXP_anovan_e-ps_tabella.pdf}
        }
        \subfloat[2048K]{
            \includegraphics[width=0.55\textwidth]{Figures/ultimi/2048K/MXP_anovan_e-ps.pdf}
        }
        \\
        
        \caption{anova n (proto + slot) Milano }
        \label{fig:XX}
\end{figure*}

\begin{figure*}[!h]
    \centering
        
         \subfloat[]{
            \includegraphics[width=0.5\textwidth]{Figures/ultimi/1024K/MRS_anovan_e-ps_tabella.pdf}
        }
        \subfloat[1024K]{
            \includegraphics[width=0.5\textwidth]{Figures/ultimi/1024K/MRS_anovan_e-ps.pdf}
        }
        \\
        
       
        
        \caption{anova n (proto + slot) Marsiglia }
        \label{fig:XX}
\end{figure*}

\begin{figure*}[!h]
    \centering
        \subfloat[]{
            \includegraphics[width=0.5\textwidth]{Figures/ultimi/400K/anova1_e-s_tabella.png}
        }
        \subfloat[400K -p wanova =XXX ]{
            \includegraphics[width=0.5\textwidth]{Figures/ultimi/400K/anova1_e-s.png}
        }
        \\
        
        \caption{anova 1 (slot) Milano}
        \label{fig:XX}
\end{figure*}


\begin{figure*}[!h]
    \centering
        \subfloat[]{
            \includegraphics[width=0.5\textwidth]{Figures/ultimi/400K/anova1_e-p_tabella.png}
        }
        \subfloat[400K -p wanova =0.001652834263777 ]{
            \includegraphics[width=0.5\textwidth]{Figures/ultimi/400K/anova1_e-p.png}
        }
        \\
        
        \caption{anova 1 (proto) Milano}
        \label{fig:XX}
\end{figure*}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/Raspberry/Energyconsumption_20minutes.pdf}
    \caption{Raspberry PI Zero 2 W, cumulative energy consumption during a 20 minute period for the different versions of the HTTP protocol.}
    \label{fig:energy}
\end{figure}

\begin{figure*}[!h]
    \centering
        \subfloat[raspberry, 1024K, MXP]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/raspberry_1024K/MXP_anovan_e-ps.pdf}
        }
        \\
    
        \subfloat[raspberry, 2048K, MXP]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/raspberry_2048K/MXP_anovan_e-ps.pdf}
        }
        \subfloat[raspberry, 4096K, MXP]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/raspberry_4096K/MXP_anovan_e-ps.pdf}
        }
        
        \caption{ANOVAN, protocol Version and ToD are the explanatory variables, power consumption is the dependent variable.}
        \label{fig:raspberry-cloudflare-anovan}
\end{figure*}


\begin{figure*}[!h]
    \centering
        \subfloat[XXXDACONTROLLAREXXXsmartphone]{
            \includegraphics[width=0.49\textwidth]{Figures/ultimi/anocova/smartphone/no_outlier.pdf}
        }
        \subfloat[XXXDARIMUOVEREXXXraspberry zero]{
            \includegraphics[width=0.49\textwidth]{Figures/ultimi/anocova/pi0Manual/no_outlier.pdf}
        }
        \\
        \subfloat[XXXDARIMUOVEREXXXraspberry Pi3 with automaticToolbox and outlier]{
            \includegraphics[width=0.49\textwidth]{Figures/ultimi/anocova/Pi3Automated/no_filtering.pdf}
        }\subfloat[XXXDARIMUOVEREXXXraspberry Pi3 with automaticToolbox and without outlier]{
            \includegraphics[width=0.49\textwidth]{Figures/ultimi/anocova/Pi3Automated/no_outlier.pdf}
        }
        \label{fig:raspberry_smartphone-cloudflare-anocova}
\end{figure*}

\input{100K}

\clearpage

\begin{figure}[!h]
    \centering
    \subfloat[Cloudflare facility code MRS (Marseille)]{
        \includegraphics[width=0.4\textwidth]{Figures/Results/Anova1/anova1_0_es.PNG}
    }
    \\
    
    

    \subfloat[Cloudflare facility code MXP (Milan)]{
       \includegraphics[width=0.4\textwidth]{Figures/Results/Anova1/anova1_1_es.PNG}
    }
    
    \caption{The impact of the slot on the energy consumption of the smartphones. The results refers to the set of experiments using a payload of 1024000 characters.}
    \label{fig:anova1_1024_slot}
\end{figure}

\begin{figure*}[!h]
    \centering
        \subfloat[400K, MXP]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/400K/MXP_anovan_e-ps.pdf}
        }
        \subfloat[1024K, MRS]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/1024K/MRS_anovan_e-ps.pdf}
        }
        \\
        \subfloat[1024K, MXP]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/1024K/MXP_anovan_e-ps.pdf}
            \label{subfig:1024}
        }
        \subfloat[2048K, MXP]{
            \includegraphics[width=0.4\textwidth]{Figures/ultimi/2048K/MXP_anovan_e-ps.pdf}
        }
        
        \caption{ANOVAN, protocol Version and ToD are the explanatory variables, power consumption is the dependent variable.}
        \label{fig:nexus-cloudflare-anovan}
\end{figure*}

\begin{figure}[!h]
    \centering
     \subfloat[XXX è comparsa una nuova facility in germaniaXXX]{
        \includegraphics[width=0.9\textwidth]{Figures/rasp/colo_4096000chars.png}
    }
    \caption{raspberry + hat, 4096000chars, 1h, periodo 20s}
    \label{fig:XX}
\end{figure}


%\input{1024K}
\clearpage

%\input{1024K_2}
\clearpage
\input{1024K_3}
\clearpage
\input{2048K}
\end{document}
